Benchmarking AI Models in Software Engineering: A Review, Search Tool, and Unified Approach for Elevating Benchmark Quality

Benchmarks are essential for unified evaluation and reproducibility. The rapid rise of Artificial Intelligence for Software Engineering (AI4SE) has produced numerous benchmarks for tasks such as code generation and bug repair. However, this proliferation has led to major challenges: (1) fragmented knowledge across tasks, (2) difficulty in selecting contextually relevant benchmarks, (3) lack of standardization in benchmark creation, and (4) flaws that limit utility. Addressing these requires a dual approach: systematically mapping existing benchmarks for informed selection and defining unified guidelines for robust, adaptable benchmark development. We conduct a review of 247 studies, identifying 273 AI4SE benchmarks since 2014. We categorize them, analyze limitations, and expose gaps in current practices. Building on these insights, we introduce BenchScout, an extensible semantic search tool for locating suitable benchmarks. BenchScout employs automated clustering with contextual embeddings of benchmark-related studies, followed by dimensionality reduction. In a user study with 22 participants, BenchScout achieved usability, effectiveness, and intuitiveness scores of 4.5, 4.0, and 4.1 out of 5. To improve benchmarking standards, we propose BenchFrame, a unified framework for enhancing benchmark quality. Applying BenchFrame to HumanEval yielded HumanEvalNext, featuring corrected errors, improved language conversion, higher test coverage, and greater difficulty. Evaluating 10 state-of-the-art code models on HumanEval, HumanEvalPlus, and HumanEvalNext revealed average pass-at-1 drops of 31.22% and 19.94%, respectively, underscoring the need for continuous benchmark refinement. We further examine BenchFrame's scalability through an agentic pipeline and confirm its generalizability on the MBPP dataset. All review data, user study materials, and enhanced benchmarks are publicly released.

==> tables/table_nl_2.tex <==
\footnotesize
\setlength{\tabcolsep}{2pt}
\renewcommand{\arraystretch}{0.7}
\begin{tabularx}{\textwidth}
    {|>{\raggedright\arraybackslash}m{1.65cm}|>{\raggedright\arraybackslash}m{3.2cm}|>{\raggedright\arraybackslash}m{3.1cm}|X|>{\raggedright\arraybackslash}m{1.5cm}|>{\raggedright\arraybackslash}m{1.3cm}|}
    \hline
    \rowcolor{lightgray}\textbf{Category} & \textbf{Name} & \textbf{Language(s)} & \textbf{No. of Problems} & \textbf{Tests} & \textbf{Task} & \textbf{Data} \\
    \hline
    \multirow{9}{*}{\makecell[1]{Code2Text}} 
        & CodeXGLUE~\cite{CodeXGLUE-2021}/ \newline CodeSearchNet~\cite{CodeSearchNet-Challenge-2019} & \footnotesize{Go, Java, JS, PHP, Python, Ruby $\rightarrow$ English} & \scriptsize{280,652 (Go), 180,253 (Java), 65,201 (JS), 39,588 (PHP), 28,588 (Python), 27,588 (Ruby)} & Labeled Pairs~\greentext{\ding{51}} & Code Summarization, Comment Generation & \github{https://github.com/microsoft/CodeXGLUE/tree/main/Code-Text/code-to-text} \\
    \cline{2-7}
        & DeepCom~\cite{DeepCom-2018} & \footnotesize{Java $\rightarrow$ English} & 588,108 & Labeled Pairs~\greentext{\ding{51}} & Code Summarization & \github{https://github.com/huxingfree/DeepCom} \\
    \cline{2-7}
        & BinSum~\cite{BinSum-2023} & \footnotesize{Binary functions (x64, x86, ARM, MIPS) $\rightarrow$ English} & 557,664 & Labeled Pairs~\greentext{\ding{51}} & Binary Code Summarization & \github{https://github.com/xinjin95/BinSum} \\
    \cline{2-7}
        & XLCoST~\cite{XLCoST-2022} & \footnotesize{C, C++, C\#, Java, JS, PHP, Python $\rightarrow$ English} & 509K \& 58K & Labeled Pairs~\greentext{\ding{51}} & Snippet \& Program Summarization & \github{https://github.com/reddy-lab-code-research/XLCoST} \\
    \cline{2-7}
        & xCodeEval~\cite{xCodeEval-2023} & \footnotesize{C, C++, C\#, Go, Java, JS, Kotlin, PHP, Python, Ruby, Rust $\rightarrow$ English} & 5,587,437 & Labeled Pairs~\greentext{\ding{51}} & Tag Classification & \github{https://github.com/ntunlp/xCodeEval/blob/main/tag_classification.md}, \huggingface{https://huggingface.co/datasets/NTU-NLP-sg/xCodeEval} \\
    \cline{2-7}
        & BIG-bench~\cite{BIG-Bench-2022} \scriptsize{\href{https://github.com/google/BIG-bench/tree/main/bigbench/benchmark_tasks/code_line_description/}{\texttt{code\_line\_description}}} & \footnotesize{Python $\rightarrow$ English} & 60 & Labeled Pairs~\greentext{\ding{51}} & Code line description & \github{https://github.com/google/BIG-bench/tree/main/bigbench/benchmark_tasks/code_line_description/} \\
    \cline{2-7}
        & Long Code Arena~\cite{long-code-arena-2024} & \footnotesize{Python $\rightarrow$ English} & 163 & Labeled Pairs~\greentext{\ding{51}} & Commit message generation & \huggingface{https://huggingface.co/datasets/JetBrains-Research/lca-commit-message-generation} \\
    \cline{2-7}
        & Long Code Arena~\cite{long-code-arena-2024} & \footnotesize{Python $\rightarrow$ English} & 216 & Labeled Pairs~\greentext{\ding{51}} & Module summarization & \huggingface{https://huggingface.co/datasets/JetBrains-Research/lca-module-summarization} \\
    \hline
\end{tabularx}
\normalsize

